Analysis of the Optimization Landscapes for Overcomplete Representation Learning

We study nonconvex optimization landscapes for learning overcomplete representations, including learning (i) sparsely used overcomplete dictionaries and (ii) convolutional dictionaries, where these unsupervised learning problems find many applications in high-dimensional data analysis. Despite the empirical success of simple nonconvex algorithms, theoretical justifications of why these methods work so well are far from satisfactory. In this work, we show these problems can be formulated as $\ell^4$-norm optimization problems with spherical constraint, and study the geometric properties of their nonconvex optimization landscapes. For both problems, we show the nonconvex objectives have benign (global) geometric structures, in the sense that every local minimizer is close to one of the target solutions and every saddle point exhibits negative curvature. This discovery enables the development of guaranteed global optimization methods using simple initializations. For both problems, we show the nonconvex objectives have benign geometric structures -- every local minimizer is close to one of the target solutions and every saddle point exhibits negative curvature -- either in the entire space or within a sufficiently large region. This discovery ensures local search algorithms (such as Riemannian gradient descent) with simple initializations approximately find the target solutions. Finally, numerical experiments justify our theoretical discoveries.

==> sections/dl-finite-landscape.tex <==
In this subsection, we argue that the geometric characteristics of $\vphiDL{\mb q}$ are similar to those of $\vphiT{\mb q}$, by demonstrating that the critical points of the finite sample objective function $\vphiDL{\mb q}$ are similar to those of the asymptotic objective function $\vphiT{\mb q}$:
\begin{itemize}[leftmargin=*]
\item \textbf{Critical points are close.} By showing finite sample concentration
\begin{align*}
	\grad \vphiDL{\mb q} \;\rightarrow\; \grad \vphiT{\mb q},\qquad \Hess \vphiDL{\mb q} \;\rightarrow\; \Hess \vphiT{\mb q},
\end{align*}
such that there is a bijection between critical points $\mb q_c$ of $\vphiDL{\mb q}$ and critical points $\ol{\mb q}_c$ of $\vphiT{\mb q}$, and $\norm{ \mb q_c - \ol{\mb q}_c }{}$ is small.
\item \textbf{Negative curvature is preserved.}	The concentration of Hessian shows that $\Hess \vphiDL{\mb q}$ has a negative eigenvalue if and only if $\Hess \vphiT{\ol{\mb q}}$ has a negative eigenvalue, and $\Hess \vphiDL{\mb q}$ is positive definite if and only if $\Hess \vphiT{\ol{\mb q}}$ is positive definite. 
\end{itemize}

Given that
\begin{align*}
	\grad \vphiDL{\mb q} \;&=\; -\frac{1}{3\theta(1-\theta)p} \mb P_{\mb q^\perp} \sum_{k=1}^p \paren{ \mb q^\top \mb A \mb x_k }^3 \paren{\mb A \mb x_k} \;=\; -\frac{1}{3\theta(1-\theta)p} \mb P_{\mb q^\perp} \paren{\mb A\mb X} \paren{ \mb X^\top \mb A^\top \mb q }^{\odot 3} \\
	\Hess \vphiDL{\mb q} \;&=\; - \frac{1}{3\theta(1-\theta)p}  \mb P_{\mb q^\perp} \brac{ 3\sum_{k=1}^p \paren{ \mb q^\top \mb A \mb x_k }^2  \mb A \mb x_k \paren{ \mb A \mb x_k }^\top - \sum_{k=1}^p \paren{ \mb q^\top \mb A \mb x_k }^4 \mb I } \mb P_{\mb q^\perp}
\end{align*}


\begin{proposition}
 We show that for all $\mb q\in \bb S^{n-1}$
 \begin{align*}
   \norm{ \grad \vphiDL{\mb q} -  \grad \vphiT{\mb q} }{} \;&\leq\; xxx \\
   \norm{ \Hess \vphiDL{\mb q} -  \Hess \vphiT{\mb q} }{} \;&\leq\; xxx 
 \end{align*}

\end{proposition}

\qq{Here, as the gradient and Hessian of $\ell^4$ is heavy-tailed, first we need to use a truncation method plus Bernstein concentration to show concentration for each $\mb q$, then we apply a union bound for covering all the points over the sphere. Or alternatively, we can use Bernoulli-Rademacher distribution to avoid this.} 





==> sections/problem.tex <==
\subsection{Basic Notations}


We use bold capital and small letters such as $\mb X$ and $\mb x$ to denote matrices and vectors, respectively. Small letters are reserved for scalars. Several specific mathematical objects we will frequently work with: $\bb S^{n-1}$ for the unit sphere in $\bb R^n$, $\bb B^n$ for the unit ball in $\bb R^n$, and $\brac{n} \doteq \Brac{1,\cdots,n}$ for positive integer. We use $\paren{\cdot}^\top$ for matrix transposition. We use superscript to index rows of a matrix, such as $\mb x^i$ for the $i$-th row of the matrix $\mb X$, and subscript to index columns, such as $\mb x_j$. For norms, $\norm{\cdot}{}$ is the usual $\ell^2$-norm for a vector and the operator norm (i.e., $\ell_2 \rightarrow \ell_2$ ) for a matrix. All
other norms will be indexed by subscript, for example the Frobenius norm $\norm{ \cdot }{F}$ for matrices and the element-wise max-norm $\norm{\cdot }{\infty}$. For any integer $p \geq 1$, the $\ell^p$-norm of a vector $\mb x \in \bb R^n$ is defined $\norm{\mb x}{p} = \paren{\sum_{k=1}^n x_k^p}^{1/p}$.
We use $x\sim \mc L$ to mean that the random variable $x$ is distributed according to the law $\mc L$. Similarly, we use  $\mb x \sim_{i.i.d.} \mc L$ to mean elements of $\mb x$ are independently and identically distributed according to the law $\mc L$. Let $\mc N$ denote the Gaussian law. Then $\mb x \sim \mc N(\mb 0, \mb I_n)$ or $\mb x \sim_{i.i.d.} \mc N(0,1)$ denotes a standard Gaussian vector. Another particular distribution of interest for this paper is the Bernoulli-Gaussian with rate $\theta$: $\Z = B \cdot G$, with $G \sim \mc N(0,1)$ and $ B \sim \mathrm{Ber}(\theta)$. We also write this compactly as  $Z\sim \mathrm{BG}(\theta) $. We frequently use indexed $c$ and $C$ for numerical constants when stating and proving technical results. The scopes of such constants are local unless otherwise noted. For a vector $\mb v \in \bb R^n$, we use 
\begin{align*}
   \mb P_{\mb v} = \frac{\mb v\mb v^\top}{ \norm{\mb v}{}^2 },\qquad \mb P_{\mb v^\perp} = \mb I - \frac{\mb v\mb v^\top}{ \norm{\mb v}{}^2 }
\end{align*}
to denote the projection operator onto $\mb v$ and orthogonal to $\mb v$, respectively. And we use $\mb v^{\odot m}$ to denote entry-wise power of order $m$, i.e., $\mb v^{\odot m} = \brac{ v_1^m, \cdots, v_n^m }^\top$.


\subsection{Riemannian derivatives}


We are solving optimization problems in \Cref{eqn:tensor-obj,eqn:odl-obj} constrained on a Riemannian manifold $\mc M = \bb S^{n-1}$. In this subsection, we give a brief introduction to manifold optimization over the sphere, and the forms of Riemannian gradient and Hessian. We refer the readers to the book \cite{absil2009} for more backgrounds. Given a point $\mb q \in S^{n-1}$, the tangent space $T_{\mb q}\bb S^{n-1}$ is defined as $T_{\mb q}\bb S^{n-1} \doteq \Brac{ \mb v \mid \mb v^\top \mb q = 0 }$. Therefore, we have the projection onto $T_{\mb q}\bb S^{n-1}$ equal to $\mb P_{\mb q^\perp}$. For a function $f(\mb q)$ defined over $\bb S^{n-1}$, we use $\grad f$ and $\Hess f$ to denote the Riemannian gradient and the Hessian of $f$, then we have
\begin{align*}
\grad f(\mb q) \doteq \mb P_{\mb q^\perp} \nabla f(\mb q), \qquad \Hess f(\mb q) \doteq \mb P_{\mb q^\perp}\paren{ \nabla^2 f(\mb q) - \innerprod{\mb q}{ \nabla f(\mb q) } \mb I } \mb P_{\mb q^\perp},
\end{align*}
where $\nabla f(\mb q)$ and $\nabla^2 f(\mb q)$ are the normal first and second derivatives in Euclidean space. In particular, for our specific function $\vphiT{\mb q}$ defined in \Cref{eqn:tensor-obj}, direct calculations reveal that
\begin{align}\label{eqn:riemannian-derviate-varphi}
   	\grad \vphiT{\mb q} &\;=\; - \mb P_{\mb q^\perp} \mb A \paren{ \mb A^\top \mb q }^{\odot 3} \;=\; - \mb P_{\mb  q^\perp} \sum_{k=1}^m \paren{ \mb a_k^\top \mb q }^3 \mb a_k, \\
   	\Hess \vphiT{\mb q} &\;=\; - \mb P_{\mb q^\perp} \brac{ 3 \mb A \diag\paren{ \paren{\mb A^\top \mb q}^{\odot 2} } \mb A^\top - \norm{ \mb A^\top \mb q }{4}^4 \mb I}\mb P_{\mb q^\perp}.
\end{align}



%\subsection{Assumptions}

%To make the problem well-posed, we study the problem under the following two assumptions of the overcomplete dictionary $\mb A \in \bb R^{n \times m}$, respectively. Similar assumptions also appear in \cite{agarwal2013exact,ge2017optimization}. 

%\paragraph{Assumption on $\mb A$.} We assume that the dictionary $\mb A$ is determined, and satisfies the $\mu$-incoherent condition.
%\begin{align}\label{eqn:assump-incoherent}
%     \frac{1}{m} \mb A \mb A^\top \;=\; \mb I,\quad \max_{ 1\leq i,j\leq m,i \not =j }\; \frac{1}{n} \abs{ \innerprod{ \mb a_i }{ \mb a_j } } \; \leq \; \mu ,\quad \frac{1}{n}\norm{ \mb a_i }{}^2 \;=\; 1, \;\; 1 \leq i \leq m.
%\end{align}
%Maybe we should consider the following (stronger condition) instead (or does the condition above imply the following?)
%\begin{align}\label{eqn:assump-incoherent-1}
%     \mb a_k \mb a_k^\top \;\approx\; \mb I,\quad \max_{ 1\leq i,j\leq m,i \not =j }\; \frac{1}{n} \abs{ \innerprod{ \mb a_i }{ \mb a_j } } \; \leq \; \mu ,\quad \frac{1}{n}\norm{ \mb a_i }{}^2 \;=\; 1, \;\; 1 \leq i \leq m.
%\end{align}
% Second, we assume that each entry of the dictionary $\mb A$ is i.i.d. random Gaussian. Notice that Assumption 2 is a special case of Assumption 1.
%\paragraph{Assumption 1: $\mu$-incoherent dictionary $\mb A$} For a given scalar $\eps$, we assume that
%\begin{align}\label{eqn:assump-incoherent}
%   \norm{\frac{1}{m} \mb A \mb A^\top - \mb I}{} \leq \eps , \qquad \max_{1\leq i,j\leq m, i\not = j} \abs{ \innerprod{\mb a_i}{\mb a_j} } \leq \mu n, \qquad \abs{ \norm{\mb a_i}{}^2 - n }\leq \eps, \; (1\leq i \leq m),
%\end{align}
%where the incoherence parameter $\mu \in \mc O\paren{ \sqrt{ \frac{ \log m }{m } } }$.

%\paragraph{Assumption 2: random dictionary $\mb A$}
%We assume that each component $\mb a_k$ of $\mb A$ is i.i.d. random Gaussian, 
%\begin{align*}
%   \mb a_k \sim_{i.i.d.} \mc N(0,1),\qquad 1\leq k\leq m.
%\end{align*}
%Note that this assumption is a special case of the previous one: with high probability over the randomness of $\mb A$, the conditions \eqref{eqn:assump-incoherent} hold for $\mb A$.  

%For the dictionary learning problem, we also make the following assumption for the sparse code $\mb X$.

%\paragraph{Sparse model of $\mb X$.} We assume that $\mb X$ follows the i.i.d. Gaussian-Bernoulli distribution with rate $\theta\in (0,1)$, i.e., $X_{ij}\sim_{i.i.d.} \mathrm{BG}(\theta)$ with
%\begin{align*}
%X_{ij} = B_{ij}G_{ij}, \quad B_{ij} \sim_{i.i.d.} \mathrm{Ber}(\theta), \quad G_{ij} \sim_{i.i.d.} \mc N(0,1),
%\end{align*}
%where $\theta \in (0,1)$ denotes the sparsity of $\mb X$. We write compactly $\mb X \sim_{i.i.d.} \mathrm{BG}(\theta)$.


==> sections/tensor-geometry.tex <==


From \Cref{eqn:DL-expectation}, we know that $\vphiDL{\mb q}$ equals to $\vphiT{\mb q}$ up to a constant when taking expectation w.r.t. $\mb X$. Precisely, we have the following.

\begin{lemma}
When $\mb X$ is i.i.d. drawn from Bernoulli Gaussian distribution as in Assumption \ref{assump:X-BG}, then we have
\begin{align*}
 	\bb E_{\mb X}\brac{ \vphiDL{\mb q}  } \; = \; \vphiT{\mb q} - \frac{\theta}{2(1-\theta)} \paren{ \frac{m}{n} }^2
\end{align*}	
\end{lemma}

The proof can be found in Appendix \ref{app:dl-asymp-landscape}. This implies that the $\vphiT{\mb q}$ can be viewed as an asymptotic version of $\vphiDL{\mb q}$ when $\mb X$ is random and $p \rightarrow + \infty$. This implies an expectation and concentration type of analysis, that we can first analyze the optimization landscape of 
\begin{align}\label{eqn:tensor-obj}
   \min_{\mb q}\; \vphiT{\mb q}\;=\; - \frac{1}{4} \norm{ \mb A^\top \mb q}{4}^4,\qquad \bb q \in \bb S^{n-1},	
\end{align}
and then turn the geometric analysis into its finite sample version $\vphiDL{\mb q}$ via measure concentration on $\mb X$.
Notice that \Cref{eqn:tensor-obj} is the 4th order overcomplete tensor problem, that has been extensively studied in xxx. \qq{More details to add for overcomplete tensor.} Our work is the first result to show global geometric for overcomplete tensor decomposition.

\begin{proposition}[Global Geometry of Overcomplete Tensor Decomposition]
  	Suppose $\mb A \in \bb R^{n \times m} $ satisfies Assumption \ref{assump:A-tight-frame}. Let $C_0>16$ be a numerical constant. Whenever
  	\begin{align*}
  	    \frac{m}{n} \;\leq \; 3\paren{ 1+ 6 C_0^{3/5} \mu^{2/5} + 6 \mu }^{-1}, 	\qquad \mu \;\leq \; \frac{1}{20},
  	\end{align*}
    the nonconvex objective $\vphiT{\mb q}$ in \Cref{eqn:tensor-obj} does not have any spurious local minimizer over the sphere. Every critical point is either a saddle point that exhibits negative curvature, or it is near one of the target solutions (e.g. $\mb a_1$),
\begin{align*}
  	\abs{\innerprod{\mb q}{ \mb a_1} } \; \geq \; 1 - 5C_0^{-3/2}.
\end{align*}
\end{proposition}

To study the optimization landscape of $\vphiT{\mb q}$, we partition the sphere $\bb S^{n-1}$ into two regions based on the function values of $\vphiT{\mb q}$. Namely, we define
\begin{align*}
   \RC \;&:=\; \Brac{ \mb q \in \bb S^{n-1} \; \mid \; -\vphiT{\mb q} \; \geq\; C_0\mu^{2/3} \norm{ \mb A^\top \mb q }{3}^2   },	\\
   \RN \;&:=\; \Brac{ \mb q \in \bb S^{n-1} \; \mid \; -\vphiT{\mb q} \; \leq\; C_0\mu^{2/3} \norm{ \mb A^\top \mb q }{3}^2   }.
\end{align*}
for some numerical constant $C_0>0$ to be determined later. In the following, we show that neither of $\RC$ and $\RN$ exhibit any spurious local minimizers. For the region $\RC(\mb q)$, where the function value $\vphiT{\mb q}$ is small, we show that all the critical points are either strict saddle points, or are near target solutions. For the region $\RN$, we show that any point $\mb q \in \RN$ exhibits strong negative curvature such that spurious local minimizer does not exist.

\paragraph{Geometric characterization of critical points in $\RC$.}
We show that all the critical points in $\mc R_2$ are either ridable saddle points, or satisfy second-order optimality condition and are close to the target solutions. 

\begin{proposition}\label{prop:dl-RC}
Let $C_0 > 16$ be a positive numerical constant. Whenever 
\begin{align*}
     \frac{m}{n} \; \leq \; \frac{C_0^{3/2}}{4},	 \quad \mu \;\leq \; \frac{1}{20},
  \end{align*}
any critical point $\mb q \in \RC$, with $\grad \vphiT{\mb q} =0$, is either a ridable (strict) saddle point, or it satisfies second-order optimality condition and is near one component, e.g., $\mb a_1$ in the sense that
\begin{align*}
  	\abs{\innerprod{\mb q}{ \mb a_1} } \; \geq \; 1 - 5C_0^{-3/2}.
\end{align*}
\end{proposition}
\begin{proof}
The proof directly follows from Appendix \ref{app:RC-proof} with $M=1$.
\end{proof}

\paragraph{Negative curvature in $\RN$.}
Finally, we show that the function $\vphiT{\mb q}$ exhibits negative curvature in the region $\RN$. Namely, the Riemannian Hessian for any points $\mb q\in \mc R_1$ is indefinite, and is negative in certain directions.
\begin{lemma}
Let $C_0\geq 4^{2/3}$ be a positive numerical constant. For any point $\mb q \in \RN$, whenever 
\begin{align*}
    \frac{m}{n} \;\leq \; 3\paren{ 1+ 6 C_0^{3/5} \mu^{2/5} + 6 \mu }^{-1},
\end{align*}
\edit{there exists at least one component $\mb a_i$ such that}
\begin{align*}
	\mb a_i^\top  \Hess \vphiT{\mb q} \mb a_i \;<\; - 4 \norm{\mb A^\top \mb q }{4}^4\norm{ \mb A^\top \mb q }{ \infty }^2.
\end{align*}
%\zz{Need to define $\mb \zeta$ or replace it by $\mb A^\top \mb q$.}
\end{lemma}

\paragraph{Remarks.} The result implies that when $n$ is large and $\mu$ is sufficiently small, for the negative curvature condition to be held, the maximum overcompleteness allowed here is roughly around $m/n \approx 3$.

\begin{proof}
The proof directly follows from Appendix \ref{app:RN-proof}.
\end{proof}





%=======

%Do we need to assume RIP condition here (stronger than incoherence)?

\begin{comment}

\subsection{Geometric Analysis}

\begin{theorem}
When $m \leq 2n$, the objective function in \Cref{eqn:tensor-obj} has no spurious local minima over the sphere $\bb S^{n-1}$.
\end{theorem}
For a given point $\mb q \in \bb S^{n-1}$, let us define a correlation vector
\begin{align*}
   \mb \zeta(\mb q) \;:=\; \mb A^\top \mb q \;\in\; \bb R^m.
\end{align*}
Let $\mb \zeta = \begin{bmatrix} \zeta_1 & \zeta_2 & \cdots & \zeta_m \end{bmatrix}^\top$, where a larger entry $\zeta_k = \mb a_k^\top \mb q$ implies higher correlation between $\mb a_k$ and $\mb q$. Let $\Brac{\zeta\order{k} }_{k=1}^m$ be the ordered entries of $\mb \zeta$ by magnitude, such that
\begin{align*}
   \abs{\zeta\order{1}} \;\geq \; \abs{ \zeta\order{2} } \;\geq \cdots \;\geq \; \abs{\zeta\order{m} }.
\end{align*}
Correspondingly, We partition the sphere into three regions
\begin{align*}
   \mc R_n \;&=\; \Brac{ \; \mb q \in \bb S^{n-1} \; \mid \; \abs{\zeta\order{2}}\;\geq \; \nu_1 \abs{\zeta\order{1}} \;}, \\
   \mc R_g \;&=\; \Brac{ \; \mb q \in \bb S^{n-1} \; \mid \;  \nu_1 \abs{\zeta\order{1}} \;\geq\; \abs{ \zeta\order{2} } \;\geq \;\nu_2  \;},  \\
   \mc R_s \;&=\; \Brac{ \; \mb q \in \bb S^{n-1} \; \mid \; \nu_2 \;\geq\; \abs{ \zeta\order{2} } \;}.
\end{align*}
Here, $\mc R_n$ denotes the region that the largest correlation $\abs{\zeta\order{1}}$ is small, where we expect negative curvatures in $\mc R_n$. On the other hand, $\mc R_s$ characterizes the region where the second largest correlation $\abs{ \zeta\order{2} }$ is small. This suggests that $\abs{ \zeta\order{1} }$ is large so that $\mb q$ is close to one of the component $\mb a\order{1}$. Within $\mc R_s$, we expect strong convexity around the ground truth. For the rest of region $\mc R_g$ over the sphere, no target solutions or saddle points exist, so that the gradient is large.

Next, we prove negative curvature, large gradient, and strong convexity in each regions of $\mc R_n$, $\mc R_g$, and $\mc R_s$, respectively. For each $\mb q \in \bb S^{n-1}$, without loss of generality, let us assume that the columns $\Brac{\mb a_k}_{k=1}^m$ of $\mb A$ are ordered such that $\abs{ \zeta_k } = \abs{ \zeta_{(k)} } \; (1\leq k \leq m)$, i.e.,
\begin{align*}
   \abs{ \zeta_1 } \;\geq \; \abs{  \zeta_2 } \; \geq \; \cdots \;\geq \; \abs{ \zeta_m }.
\end{align*}



\paragraph{Negative Curvature.} First, we show that the function exhibits negative curvature in the region $\mc R_n$.

\begin{lemma}
When $m \leq 3 \paren{ \nu_1^2 - 6\mu }n $, there exists some direction $\mb v $ such that
\begin{align*}
   \mb v^\top \Hess \vphiT{\mb q} \mb v \;\leq\; - \nu_2^2 \zeta_1^4 \norm{\mb v}{}^2
\end{align*}
for all 
\begin{align*}
\mb q \in \mc R_n \;&=\; \Brac{ \; \mb q \in \bb S^{n-1} \; \mid \; \abs{\zeta_2}\;\geq \; \nu_1 \abs{\zeta_1} \;},	
\end{align*}
with $\nu_1 \in (0,1)$.
\end{lemma}

\begin{proof}
 Without loss of generality, we assume that $ \norm{ \mb v }{} = 1$. Let us choose our direction $\mb v$ as a linear combination of $\mb a_1$ and $\mb a_2$, i.e., $\mb v =  \alpha_1 \mb a_1 + \alpha_2 \mb a_2$ with $ \alpha_1,\alpha_2 \in (-1,1)$. Since $\mathrm{span}\paren{ \mb a_1,\mb a_2 } \bigcap  \mathrm{span}\paren{\mb q}^\perp \not = \emptyset $, there exist $\alpha_1,\alpha_2\in (-1,1)$ such that $\mb v \perp \mb q $. Therefore, we have
\begin{align*}
   \alpha_1^2 + \alpha_2^2  \;=\; 1 - 2 \alpha_1 \alpha_2 \innerprod{\mb a_1}{\mb a_2} \quad\Longrightarrow\quad  1- 2\mu  \leq \alpha_1^2 + \alpha_2^2 \leq 1 + 2\mu.
\end{align*}
Thus, we have 
\begin{align*}
   	\mb v^\top \Hess \vphiT{\mb q} \mb v \;&=\; - 3 \mb v^\top \mb P_{\mb q^\perp} \mb A \diag\paren{ \mb \zeta^{\odot 2}  }  \mb A^\top \mb P_{\mb q^\perp} \mb v + \norm{ \mb \zeta }{4}^4 \cdot \norm{ \mb P_{\mb q^\perp} \mb v }{}^2 \\
   	\;&=\; -3 \mb v^\top \mb A \diag\paren{ \mb \zeta^{\odot 2}  }  \mb A^\top\mb v + \norm{ \mb \zeta }{4}^4 \\
   	\;&=\; -3  \innerprod{\mb a_1}{ \mb v}^2 \zeta_1^2 - 3 \innerprod{\mb a_2}{ \mb v}^2 \zeta_2^2 - 3 \sum_{k=3}^m \innerprod{\mb a_k}{ \mb v}^2 \zeta_k^2 + \norm{ \mb \zeta }{4}^4 \\
   	\; &\leq\; -3  \innerprod{\mb a_1}{ \mb v}^2 \zeta_1^2 - 3 \innerprod{\mb a_2}{ \mb v}^2  \nu_1^2 \zeta_1^2 + \zeta_1^4 + \sum_{k=2}^m \zeta_k^4
\end{align*}
By incoherence, we have
\begin{align*}
   \innerprod{\mb a_1}{ \mb v}^2 \;&=\; \alpha_1^2 + \alpha_2^2 \innerprod{\mb a_1}{ \mb a_2}^2 + 2 \alpha_1 \alpha_2 \innerprod{\mb a_1}{ \mb a_2}, \\
   \innerprod{\mb a_2}{ \mb v}^2 \;&=\; \alpha_2^2 + \alpha_1^2 \innerprod{\mb a_1}{ \mb a_2}^2 + 2 \alpha_1 \alpha_2 \innerprod{\mb a_1}{ \mb a_2},
\end{align*}
so that
\begin{align*}
   	\innerprod{\mb a_1}{ \mb v}^2 + \innerprod{\mb a_2}{ \mb v}^2 \;&=\; \alpha_1^2 + \alpha_2^2 + \innerprod{\mb a_1}{ \mb a_2}^2 \paren{\alpha_1^2 + \alpha_2^2} + 4 \alpha_1\alpha_2 \cdot \innerprod{\mb a_1}{ \mb a_2} \\
   	 \;&\geq\; 1 - 2\mu - 4 \mu \;=\; 1- 6 \mu.
\end{align*}
On the other hand, by the fact that $\norm{\mb \zeta}{}^2 =\frac{m}{n}$, we have
\begin{align*}
   \sum_{k=2}^m \zeta_k^4 \;\leq\; \zeta_2^2 \sum_{k=2}^m \zeta_k^2  \;=\;  \zeta_2^2 \paren{ \frac{m}{n} - \zeta_1^2 },
\end{align*}
Therefore, we have
\begin{align*}
	\mb v^\top \Hess \vphiT{\mb q} \mb v \;&\leq \; -3 \paren{ \mb a_1^\top \mb v }^2 \zeta_1^2 - 3 \paren{ \mb a_2^\top \mb v }^2 \nu_1^2\zeta_1^2 + \zeta_2^2 \paren{ \frac{m}{n} - \zeta_1^2 }  \\
	\;&\leq \; -3 \brac{ \paren{ \mb a_1^\top \mb v }^2 + \paren{ \mb a_2^\top \mb v }^2 } \zeta_1^2 \;+\; 3\paren{1-\nu_1^2} \innerprod{\mb a_2}{\mb v}^2 \zeta_1^2 \;+\;  \zeta_2^2 \paren{\frac{m}{n} - \zeta_1^2} \\
	\;&\leq\; - 3 \paren{ 1- 6\mu} \zeta_1^2 \;+\; \frac{m}{n} \zeta_2^2  +3 \paren{1-\nu_1^2}\zeta_1^2 - \zeta_1^2\zeta_2^2.
\end{align*}
Therefore, whenever
\begin{align*}
   \frac{m}{n} \leq 3 \paren{ \nu_1^2 - 6\mu },	
\end{align*}
we have 
\begin{align*}
	\mb v^\top \Hess \vphiT{\mb q} \mb v \;&\leq \; - c \zeta_1^2.
\end{align*}


%the bound above can be tightened a bit (I used the loosest approach). How to lower bound
%\begin{align*}
%   \sum_{k=3}^m \paren{ \mb a_k^\top \mb v }^2 \zeta_k^2 \;\geq\; xxx   \;\;? 	
%\end{align*}

\end{proof}




%We could further partition $\mc R_n$ based on function value 
%\begin{align*}
%   \mc L(\eps) \;&:=\; \Brac{ \; \mb q \in \bb S^{n-1} \;\mid\; -\norm{\mb A^\top \mb q}{4}^4 \;\leq\; -3\cdot \frac{m}{n^2}\; +\; \eps \;}, \\
%   \mc L^c(\eps) \;&:=\; \Brac{ \; \mb q \in \bb S^{n-1} \;\mid\; -\norm{\mb A^\top \mb q}{4}^4 \;>\; -3\cdot \frac{m}{n^2}\; +\; \eps \;}.
%\end{align*}
% to refine the bounds for overcompleteness.

\paragraph{Large Gradient.} We prove the following

\begin{lemma}
There exists some direction $\mb v$ such that 
\begin{align*}
   \innerprod{\mb v}{ - \grad \vphiT{\mb q} } \;\geq\; c\; xx
\end{align*}
for all 
$$ \mb q \;\in\; \mc R_g \;=\; \Brac{ \; \mb q \in \bb S^{n-1} \; \mid \;  \nu_1 \abs{\zeta_1} \;\geq\; \abs{ \zeta_2 } \;\geq \;\nu_2  \;}$$.
\end{lemma}

\begin{proof}
Choose $\mb v = - \sign\paren{\zeta_1 }  \mb a_1$, we have
\begin{align*}
   \mb v^\top \grad \vphiT{\mb q} \;&=\;   \sign\paren{\zeta_1 } \sum_{k=1}^m \zeta_k^3 \paren{ \mb a_1^\top \mb P_{\mb q^\perp} \mb a_k }\\
   \;&=\; \abs{\zeta_1}^3 \norm{ \mb P_{\mb q^\perp} \mb a_1 }{}^2 +  \sign\paren{\zeta_1 }  \sum_{k=2}^m \zeta_k^3 \paren{ \mb a_1^\top \mb P_{\mb q^\perp} \mb a_k } \\
   \;&=\; \abs{\zeta_1}^3 - \abs{\zeta_1}^5  + \sign\paren{\zeta_1 }  \sum_{k=2}^m \zeta_k^3 \innerprod{ \mb a_1 }{ \mb a_k } - \abs{\zeta_1} \sum_{k=2}^m \zeta_k^4   \\
   \;& \geq\; 
\end{align*}	
By using the fact that
\begin{align*}
   \norm{ \mb \zeta }{4}^4 \; \leq \; \zeta_1^4 + \zeta_2^2 \sum_{k=2}^m \zeta_k^2 \;=\; \zeta_1^4 + \zeta_2^2 \paren{ \frac{m}{n} - \zeta_1^2 }, 
\end{align*}
we obtain
\begin{align*}
   \mb v^\top \grad \vphiT{\mb q} \;&\geq\; \zeta_1 \brac{  \zeta_1^2 - \nu_1 \mu \paren{ \frac{m}{n} - \zeta_1^2 } - \zeta_1^4 - \nu_1^2 \zeta_1^2 \paren{ \frac{m}{n} - \zeta_1^2 } }	 \\
   \;&=\; \zeta_1 \brac{ \paren{1+ \nu_1 \mu - \frac{m}{n}\nu_1^2} \zeta_1^2 - \paren{1- \nu_1^2}\zeta_1^4 -  \nu_1 \mu\frac{m}{n} }
\end{align*}



\end{proof}


\paragraph{Strong Convexity.} We need to show that

\begin{lemma}
For all $\mb v \perp \mb q $,
\begin{align*}
   \mb v^\top \Hess \vphiT{\mb q} \mb v  \;\geq\; C\cdot \zeta_1^2,
\end{align*}
for all 
\begin{align*}
	\mb q \in \mc R_s \;=\; \Brac{ \; \mb q \in \bb S^{n-1} \; \mid \; \nu_2 \;\geq\; \abs{ \zeta_2 } \;},
\end{align*}
where $\nu_2 =  $
\end{lemma}

\begin{proof}
For all $\mb v \perp \mb q $ with $\mb v \in \bb S^{n-1}$, we have
\begin{align*}
   	\mb v^\top \Hess \vphiT{\mb q} \mb v \;&=\; - 3 \mb v^\top \mb P_{\mb q^\perp} \mb A \diag\paren{ \mb \zeta^{\odot 2}  }  \mb A^\top \mb P_{\mb q^\perp} \mb v + \norm{ \mb \zeta }{4}^4 \cdot \norm{ \mb P_{\mb q^\perp} \mb v }{}^2 \\
   	\;&=\; \norm{ \mb \zeta }{4}^4 - 3 \sum_{k=1}^m \zeta_k^2 \paren{ \mb a_k^\top \mb v }^2  \\
   	\;&=\; \norm{ \mb \zeta }{4}^4 - 3 \zeta_1^2 \paren{ \mb a_1^\top \mb v }^2 - 3 \sum_{k=2}^m \zeta_k^2 \paren{ \mb a_k^\top \mb v }^2 \\
   	\;&\geq\; \norm{ \mb \zeta }{4}^4 - 3 \zeta_1^2 \paren{ \mb a_1^\top \mb v }^2 - 3 \zeta_2^2 \cdot \sum_{k=2}^m \paren{ \mb a_k^\top \mb v }^2 \\
   	\;&= \;  \norm{ \mb \zeta }{4}^4 - 3 \zeta_1^2 \paren{ \mb a_1^\top \mb v }^2 - 3 \zeta_2^2 \cdot \paren{ \frac{m}{n}  - \paren{ \mb a_1^\top \mb v }^2 }\\
   	\;&\geq \; \norm{ \mb \zeta }{4}^4 - 3 \zeta_1^2 \paren{ \mb a_1^\top \mb v }^2 - 3 \frac{m}{n}  \nu_2^2    
\end{align*}
By tight frame, for all $\mb v \in \bb S^{n-1}$, by the fact that $\mb A\mb A^\top = \mb a_1\mb a_1^\top \;+\; \sum_{k=2}^m \mb a_k \mb a_k^\top \;=\; \frac{m}{n} \mb I$, we have
\begin{align*}
   \paren{ \mb a_1^\top \mb v }^2 \;=\; \frac{m}{n} - \sum_{k=2}^m \paren{ \mb a_k^\top \mb v }^2 ,\qquad \zeta_1^2 \;=\; \frac{m}{n} - \sum_{k=2}^m \zeta_k^2\;\geq\; \frac{m}{n} - (m-1) \nu_2^2
\end{align*}
Since for all $\mb q \in \bb S^{n-1}$,
\begin{align*}
   \norm{\mb P_{\mb q^\perp} \mb a_1}{}^2 \;&=\; \norm{\mb a_1}{}^2 - \norm{\mb P_{\mb q} \mb a_1}{}^2\;=\; 1 - \zeta_1^2, \\
   \paren{ \mb a_1^\top \mb v }^2\;&\leq\; \norm{\mb P_{\mb q^\perp} \mb a_1}{}^2 \;\leq\; 1 - \zeta_1^2 \;\leq\; 1 - \frac{m}{n} + (m-1) \nu_2^2,
\end{align*}
we obtain 
\begin{align*}
   \mb v^\top \Hess \vphiT{\mb q} \mb v \; &\geq \; \zeta_1^4 - 3 \zeta_1^2 \underbrace{\paren{ 1 - \frac{m}{n} + (m-1) \nu_2^2 } }_{\text{should be small}} - 3 \frac{m}{n} \nu_2^2\;\geq\; C \zeta_1^2
\end{align*}
for properly small $\nu_2^2 \in O(1/n)$.





\end{proof}


\end{comment}





%=============

%\noindent 
%We can do a different partition with
%\begin{align*}
%   \mc R_1 \;&=\; \Brac{ \mb q \in \bb S^{n-1} \; \mid \; \norm{ \mb \zeta }{4}^4 \; \leq\; C_0\mu^{2/3} \norm{ \mb \zeta }{3}^2   }	\\
%   \mc R_2 \;&=\; \Brac{ \mb q \in \bb S^{n-1} \; \mid \; \norm{ \mb \zeta }{4}^4 \; \geq\; C_0\mu^{2/3} \norm{ \mb \zeta }{3}^2   }
%\end{align*}
%Thus, we have
%\begin{align*}
%    &\mb a_1^\top  \Hess \vphiT{\mb q} \mb a_1 \\
%    \leq\;& -3 \norm{ \mb \zeta }{\infty}^2 +6 \norm{ \mb \zeta }{ \infty }^4 +6 \mu \norm{ \mb \zeta }{\infty } \abs{\norm{\mb \zeta}{3}^3 } - 4  \norm{ \mb \zeta }{\infty}^2 \norm{ \mb \zeta }{4}^4 + \norm{ \mb \zeta }{4}^4 \\
%    \leq\;& \norm{ \mb \zeta }{ \infty }^2 \paren{ -3  +6 \norm{ \mb \zeta }{ \infty }^2 + 6 \mu \norm{ \mb \zeta}{}^2-4 \norm{ \mb \zeta }{4}^4  + \norm{ \mb \zeta }{}^2  } \\
%     \leq\;& \norm{ \mb \zeta }{ \infty }^2 \paren{ -3  +6 \norm{ \mb \zeta }{ \infty }^2 + 6 \mu \frac{m}{n} -4 \norm{ \mb \zeta }{4}^4  + \frac{m}{n}  }
%\end{align*}
%where for the last inequality, we used the fact that $ \norm{\mb \zeta}{ 4}^4 \leq \norm{\mb \zeta}{ \infty }^2 \norm{\mb \zeta}{}^2  $ and $\norm{ \mb \zeta }{}^2 = \frac{m}{n}$. Moreover, we observe
%\begin{align*}
%   \norm{ \mb \zeta }{\infty}^2 \;&\leq\; \norm{ \mb \zeta}{4}^2 \;\leq\; C_0^{1/2} \mu^{1/3} \norm{ \mb \zeta }{3}	 \\
%   \norm{\mb \zeta}{3} \;&=\; \paren{ \sum_{k=1}^m \zeta_k^3 }^{1/3}\;\leq\; \norm{\mb \zeta}{\infty }^{1/3} \paren{\frac{m}{n}}^{1/3}.
%\end{align*}
%Thus, we obtain
%\begin{align*}
%   	 \norm{ \mb \zeta }{\infty}^2 \;\leq\; C_0^{1/2} \mu^{1/3}  \norm{\mb \zeta}{\infty }^{1/3} \paren{\frac{m}{n}}^{1/3} \quad \Longrightarrow \quad \norm{ \mb \zeta }{\infty}^2 \;\leq\; C_0^{3/5} \paren{ \mu \frac{m}{n} }^{2/5}. 
%\end{align*}
%Hence, we have
%\begin{align*}
%   	\mb a_1^\top  \Hess \vphiT{\mb q} \mb a_1 
%\;&\leq\; \norm{ \mb \zeta }{ \infty }^2 \paren{ -3  +6 C_0^{3/5} \paren{ \mu \frac{m}{n} }^{2/5} + 6 \mu \frac{m}{n} -4 \norm{ \mb \zeta }{4}^4  + \frac{m}{n}  } \\
%\;&\leq\; -4 \norm{ \mb \zeta }{4}^4 \norm{ \mb \zeta }{ \infty }^2,
%\end{align*}
%given that
%\begin{align*}
%    \frac{m}{n} \;\leq \; 3\paren{ 1+ 6 C_0^{3/5} \mu^{2/5} + 6 \mu }^{-1} .
%\end{align*}

%=====





%For a given point $\mb q \in \bb S^{n-1}$, without loss of generality, let us assume that the columns $\Brac{\mb a_k}_{k=1}^m$ of $\mb A$ are ordered as such
%\begin{align*}
%   \abs{\mb a_1^\top \mb q} \;\geq\; \abs{ \mb a_2^\top \mb q } \;\geq\; \cdots \;\geq\; \abs{\mb a_m^\top \mb q }.
%\end{align*}


%\subsection{Approach 1 -- Direction Calculation}

%We partition the space into two regions
%\begin{align}
% 	\mc R_1 \;&=\; \Brac{ \mb q \in \bb S^{n-1} \;\mid\; \norm{ \mb A^\top \mb q }{ \infty }^2 \;\leq\; \frac{1}{24} - 2 \mu  } \\
% 	\mc R_2 \;&=\; \bb S^{n-1} \setminus \mc R_1.
%\end{align}


%\paragraph{Negative Curvature in $\mc R_1$.} We show the following result. 

%\begin{lemma}
%Given any point $\mb q \in \mc R_1$, we have
%\begin{align*}
%   \mb a_1^\top \Hess \vphiT{\mb q} \mb a_1 \;\leq \; xxx
%\end{align*}
%\end{lemma}

%\begin{proof}
%Let us write $\mb \zeta = \mb A^\top \mb q$, then we observe
%\begin{align*}
%    \mb a_1^\top \Hess \vphiT{\mb q} \mb a_1 \;= \;
%\end{align*}

%\end{proof}


\begin{comment}

\subsection{Approach 2 -- Sum of Squares bound}
Given
\begin{align*}
   \vphiT{\mb q} = - \norm{\mb A^\top \mb q}{4}^4,	
\end{align*}
we partition the optimization landscape based on the function value $\vphiT{\mb q}$ into two regions,
\begin{align*}
   \mc L \;&:=\; \Brac{ \; \mb q \in \bb S^{n-1} \;\mid\;  \vphiT{\mb q} \;\leq\; -C\cdot \frac{m}{n^2} \;}, \\
   \mc L^c \;&:=\; \Brac{ \; \mb q \in \bb S^{n-1} \;\mid\; \vphiT{\mb q} \;>\; -C\cdot \frac{m}{n^2} \;}.
\end{align*}
We show that the function has no spurious local minima in both the sets $\mc L$. 


\paragraph{SOS for negative curvature in $\mc L(\eps)$.} Let $\mb \zeta = \mb A^\top \mb q$, we prove negative curvature by showing that
\begin{align*}
	g(\mb q) \;:=\;  \mb a_1^\top \Hess \varphi(\mb q) \mb a_1 \;\leq \; - c \norm{\mb a_1}{}^2,
\end{align*}
where
\begin{align*}
    g(\mb q) \;=\;& - \mb a_1^\top \mb P_{\mb q^\perp} \brac{ 3 \mb A \diag\paren{ \mb \zeta^{ \odot 2 }  }  \mb A^\top - \norm{ \mb \zeta }{4}^4 \mb I }  \mb P_{\mb q^\perp} \mb a_1 \\
    \;=\;& - 3 \sum_{k=1}^m \paren{ \mb a_k^\top \mb P_{\mb q^\perp} \mb a_1 }^2 \zeta_k^2 \;+\;  \norm{ \mb P_{\mb q^\perp} \mb a_1 }{}^2 \norm{\mb \zeta}{4}^4 \\
    \;=\;& - 3 \norm{  \mb P_{\mb q^\perp} \mb a_1 }{}^4 \zeta_1^2 - 3 \sum_{k=2}^m \zeta_k^2 \paren{ \mb a_k^\top \mb P_{\mb q^\perp} \mb a_1 }^2 + \norm{ \mb P_{\mb q^\perp} \mb a_1 }{}^2 \norm{\mb \zeta}{4}^4 \\
    \;=\;& - 3 \norm{  \mb P_{\mb q^\perp} \mb a_1 }{}^4 \zeta_1^2 + \norm{ \mb P_{\mb q^\perp} \mb a_1 }{}^2 \norm{\mb \zeta}{4}^4 - 3 \sum_{k=2}^m \zeta_k^2 \paren{ \mb a_k^\top \mb P_{\mb q^\perp} \mb a_1 }^2  \\
    &+ \frac{3}{n}  \sum_{k=2}^m \zeta_k^2 \norm{ \mb P_{\mb q^\perp} \mb a_1 }{}^2 - \frac{3}{n} \sum_{k=2}^m \zeta_k^2 \norm{ \mb P_{\mb q^\perp} \mb a_1 }{}^2 \\
    \;=\;& - \norm{  \mb P_{\mb q^\perp} \mb a_1 }{}^2  \brac{ 3 \zeta_1^2 \norm{  \mb P_{\mb q^\perp} \mb a_1 }{}^2 - \zeta_1^4 + \frac{3}{n}  \sum_{k=2}^m \zeta_k^2  -   \sum_{k=2}^m \zeta_k^4 }  \\
     & +  3 \sum_{k=2}^m \zeta_k^2 \paren{ \frac{1}{n} \norm{ \mb P_{\mb q^\perp} \mb a_1  }{}^2 - \paren{ \mb a_k^\top \mb P_{\mb q^\perp} \mb a_1 }^2  }  \\
     \;=\;&  - \norm{  \mb P_{\mb q^\perp} \mb a_1 }{}^2 \underbrace{ \brac{ 3 \zeta_1^2 - 3 \zeta_1^4 - \norm{\mb \zeta}{4}^4 + \frac{3}{n} \norm{ \mb \zeta }{}^2- \frac{3}{n} \zeta_1^2 } }_{g \paren{ \mb \zeta } } \\
     & +  3 \sum_{k=2}^m \zeta_k^2 \paren{ \frac{1}{n} \norm{ \mb P_{\mb q^\perp} \mb a_1  }{}^2 - \paren{ \mb a_k^\top \mb P_{\mb q^\perp} \mb a_1 }^2  }
\end{align*} 
We want a \emph{tight} upper bound for
\begin{align*}
    3 \sum_{k=2}^m \zeta_k^2 \paren{ \frac{1}{n} \norm{ \mb P_{\mb q^\perp} \mb a_1  }{}^2 - \paren{ \mb a_k^\top \mb P_{\mb q^\perp} \mb a_1 }^2  }.
\end{align*}
A simple bound produces
\begin{align*}
    3 \sum_{k=2}^m \zeta_k^2 \paren{ \frac{1}{n} \norm{ \mb P_{\mb q^\perp} \mb a_1  }{}^2 - \paren{ \mb a_k^\top \mb P_{\mb q^\perp} \mb a_1 }^2  } \; \leq\; 3  \frac{m}{n} \zeta_2^2,
\end{align*}
or
\begin{align*}
    3 \sum_{k=2}^m \zeta_k^2 \paren{ \frac{1}{n} \norm{ \mb P_{\mb q^\perp} \mb a_1  }{}^2 - \paren{ \mb a_k^\top \mb P_{\mb q^\perp} \mb a_1 }^2  } \; &\leq\; \frac{3}{n} \norm{ \mb P_{\mb q^\perp} \mb a_1  }{}^2 \paren{ \sum_{k=2}^m \zeta_k^2 } \cdot  \max_{2\leq k \leq m} \abs{ 1 + n\paren{ \mb a_k^\top \frac{\mb P_{\mb q^\perp} \mb a_1}{ \norm{ \mb P_{\mb q^\perp} \mb a_1  }{}  } }^2 }  \\
    \; &\leq\; \frac{3}{n} \norm{ \mb P_{\mb q^\perp} \mb a_1  }{}^2 \paren{ \sum_{k=2}^m \zeta_k^2 } \cdot  \max_{2\leq k \leq m} \brac{ 1 + 4 n\paren{\mu^2 + \zeta_1^4 } }
\end{align*}

Let us define
\begin{align}
  g(\mb \zeta) \;:=\; 3 \zeta_1^2 - 3 \zeta_1^4 - \norm{\mb \zeta}{4}^4 + \frac{3}{n} \norm{ \mb \zeta }{}^2- \frac{3}{n} \zeta_1^2  \label{eqn:g-zeta}
\end{align}
We want to show positivity of $g(\mb \zeta)-t$ for some $t>0$, over the set
\begin{align}
   \mc S(\mb \zeta) \;:=\;	\Brac{ \mb \zeta \in \bb R^m \; \mid\; \norm{ \mb \zeta }{}^2 = \frac{m}{n},\; C\frac{m}{n^2} - \norm{ \mb \zeta }{4}^4 \geq 0,\; \zeta_1^2 - \zeta_k^2 \geq 0 \;(2\leq k\leq m) }.
\end{align}
By Putninar's positivellentz, for $g(\mb \zeta) -t $ to be nonnegative over the set $\mc S(\mb \zeta)$, it is necessary and sufficient to have
\begin{align}\label{eqn:g-sos}
  g(\mb \zeta) -t \;=\; \sigma_0(\mb \zeta) + h(\mb \zeta)\paren{  \norm{ \mb \zeta }{}^2 - \frac{m}{n} } + \sigma_1(\mb \zeta) \paren{ C\frac{m}{n^2} - \norm{\mb \zeta}{4}^4 } + \sum_{k=2}^m \sigma_k(\mb \zeta) \paren{ \zeta_1^2 - \zeta_k^2 },
\end{align}
where $h(\mb \zeta)$ is a polynomial, and $\Brac{ \sigma_k(\mb \zeta) }_{k=0}^m$ are sum of squares polynomials. One set of possible solutions for $h(\mb \zeta)$ and $\Brac{ \sigma_k(\mb \zeta) }_{k=0}^m$ is
\begin{align*}
   \sigma_k(\mb \zeta) \;&=\; c_1 \zeta_k^2,\qquad 2 \leq k \leq m, \\
   \sigma_1(\mb \zeta) \;&=\; c_2 + c_3 \zeta_1^2 \\
   h(\mb \zeta) \;&=\; c_4 + c_5 \zeta_1^2 + c_6 \norm{\mb \zeta}{}^2 \\
   c_1 + c_2 &= 1,\qquad c_1,\;c_2,\;c_3\;\geq\;0,
\end{align*}
where $c_1,\;c_2,\;c_3,\;,c_4,\;c_5$ and $c_6$ are parameters to be chosen. Plugging the solution above back into \Cref{eqn:g-sos}, we obtain
\begin{align*}
   \sigma_0(\mb \zeta) \;=\;& \underbrace{\paren{ c_4 \frac{m}{n} - c_2 C \frac{m}{n} -t }}_{a_0} + \underbrace{\paren{ 3 - \frac{3}{n} +c_5 \frac{m}{n} - c_3 C \frac{m}{n} } }_{a_1} \zeta_1^2 + \underbrace{\paren{ \frac{3}{n} - c_4 + c_6 \frac{m}{n} } }_{a_2} \norm{\mb \zeta}{}^2 + \underbrace{\paren{-c_1 - c_5}}_{a_3} \zeta_1^2 \norm{ \mb \zeta }{}^2 \\
   & -3\zeta_1^4+ (c_1+c_2-1) \norm{\mb \zeta}{4}^4  - c_6 \norm{\mb \zeta}{}^4  + c_3 \zeta_1^2 \norm{ \mb \zeta }{4}^4.
\end{align*}
Constructing a sum of squares polynomial $\sigma_0(\mb \zeta)$ such that $t$ is maximized can be reduced to solve a SDP problem. Notice that the structure of $\sigma_0(\mb \zeta)$ has permutation symmetry --- the permutation of orders of $\paren{ \zeta_2,\zeta_3,\cdots, \zeta_m }$ produces the same $\sigma_0(\mb \zeta)$. By utilizing this structure, we construct a vector of monomials and coefficients,
\begin{align*}
   [\mb \zeta ]_n\; =\; \begin{bmatrix}
 	1 \\ \zeta_1 \\ \wh{\zeta}^2 \\ \zeta_1 \wh{\zeta}^2 \\ \zeta_1^3 \end{bmatrix},\qquad \mb c \;=\; \begin{bmatrix}
 	c_1 \\ c_2 \\ \vdots \\ c_6
 \end{bmatrix},
\end{align*}
where $\wh{\zeta}$ denotes $\zeta_k\;(2\leq k\leq m)$. Let $\mb Q(\mb c)$ to be a symmetric matrix of coefficients $\mb c$, such that 
\begin{align*}
    \sigma_0(\mb \zeta) \;=\; 	[\mb \zeta ]_n^\top\; \mb Q \; [\mb \zeta ]_n,\qquad \mb Q \succeq \mb 0.
\end{align*}
This leads to the following SDP problem
\begin{align*}
   &\max_{t,\mb Q,\mb c} \; t , \\
   & Q_{11} \;=\; c_4 \frac{m}{n} - c_2 C \frac{m}{n} -t,\quad Q_{22} \;=\; 3 - \frac{3}{n} +c_5 \frac{m}{n} - c_3 C \frac{m}{n}, \\
   & 2Q_{13} \;=\; \paren{\frac{3}{n} - c_4 + c_6 \frac{m}{n} } m ,\; Q_{33}\;=\; - c_6 m^2,\; 2Q_{24} \;=\; -(m-1)(c_1+c_5),  \\
   &  2Q_{25} \;=\; -c_1 - c_5 -3 ,\;Q_{44} \;=\; (m-1) c_3,\; Q_{55}\;=\; c_3, \\
   & Q_{12} \;=\; Q_{14} \;=\; Q_{15} \;=\; Q_{23} \;=\; Q_{34} \;=\; Q_{35} \;=\; Q_{45}\;=\; 0, \\
   & \mb Q \succeq \mb 0,\; c_1 + c_2 - 1 \;=\;0,\;c_1\;\geq\; 0,\;c_2\;\geq\;0,\;c_3 \;\geq \; 0.
\end{align*}

The numerical observation leads to the SoS construction of $\sigma_0(\mb \zeta)$ in the following form,
\begin{align*}
   \sigma_0(\mb \zeta) \;=\;& - c_6 \norm{ \mb \zeta }{}^4 + \paren{ \frac{3}{n} - c_4 + c_6 \frac{m}{n} } \norm{ \mb \zeta }{}^2 + \paren{ c_4 \frac{m}{n} - c_2 C\frac{m}{n} -t }  \\
   & + c_3 \zeta_1^6 - \paren{ c_1 + c_5 + 3 } \zeta_1^4 + \frac{ \paren{ c_1 + c_5 + 3 }^2  }{4c_3}\zeta_1^2 + \zeta_1^2 \sum_{k=2}^m \brac{ c_3 \zeta_k^4 - \paren{c_1+c_5} \zeta_k^2 +  \frac{ \paren{ c_1+c_5 }^2 }{4c_3}  } \\
   & + \zeta_1^2 \brac{ 3 - \frac{3}{n} + c_5 \frac{m}{n} - c_3 C\frac{m}{n} - (m-1)\frac{ \paren{ c_1+c_5 }^2 }{4c_3} - \frac{ \paren{ c_1 + c_5 + 3 }^2  }{4c_3} } \\
   \;=\;& - c_6 \paren{ \norm{ \mb \zeta }{}^2 - \frac{m}{n}  }^2 +  \brac{  c_4 \frac{m}{n} - c_2 C\frac{m}{n} -t + c_6 \paren{\frac{m}{n}}^2 }  \\
   & + c_3 \zeta_1^2\paren{ \zeta_1^2 - \frac{ c_1 + c_5 + 3   }{2c_3} }^2 + c_3 \zeta_1^2 \sum_{k=2}^m \paren{ \zeta_k^2 - \frac{c_1+c_5 }{2c_3} }^2   \\
   & + \zeta_1^2 \brac{ 3 - \frac{3}{n} + c_5 \frac{m}{n} - c_3 C\frac{m}{n} - (m-1)\frac{ \paren{ c_1+c_5 }^2 }{4c_3} - \frac{ \paren{ c_1 + c_5 + 3 }^2  }{4c_3} }.
\end{align*}

A sufficient condition for $\sigma_0(\mb \zeta)$ to be sum of squares is 
\begin{align}
   2c_6 \frac{m}{n} \;&=\; \frac{3}{n} - c_4 + c_6 \frac{m}{n}	\label{eqn:cond-1} \\
   c_4 \frac{m}{n} - c_2 C\frac{m}{n} -t + c_6 \paren{\frac{m}{n}}^2\;&\geq \; 0, \quad c_6\;\leq\; 0, \label{eqn:cond-2} \\
   c_1 + c_2 -1 \;&=\; 0,\quad c_1 \geq 0,\;c_2\;\geq \;0,\;c_3\;\geq \;0, \label{eqn:cond-3} \\
    3 - \frac{3}{n} + c_5 \frac{m}{n} - c_3 C\frac{m}{n} - (m-1)\frac{ \paren{ c_1+c_5 }^2 }{4c_3} - \frac{ \paren{ c_1 + c_5 + 3 }^2  }{4c_3} \;&\geq \; 0. \label{eqn:cond-4}
\end{align}
Combining \Cref{eqn:cond-1} and \Cref{eqn:cond-2}, we have
\begin{align*}
	c_6 \frac{m}{n} \;&=\; \frac{3}{n} - c_4,\quad \frac{3m}{n^2} -t \;\geq\; c_2 C \frac{m}{n}.
\end{align*}
Moreover, by utilizing \Cref{eqn:cond-3}, we obtain
\begin{align*}
    c_1 \;\geq \; 1 - \frac{ 3m/n^2 - t }{ C m/n }	
\end{align*}
In addition, \Cref{eqn:cond-4} implies that
\begin{align*}
    3 \;\geq \; \frac{3}{n} 	+ \frac{ \paren{ c_1 + c_5 + 3 }^2  }{4c_3}
\end{align*}


\end{comment}


%Maybe we should consider the following (stronger condition) instead (or does the condition above imply the following?)
%\begin{align}\label{eqn:assump-incoherent-1}
%     \mb a_k \mb a_k^\top \;\approx\; \mb I,\quad \max_{ 1\leq i,j\leq m,i \not =j }\; \frac{1}{n} \abs{ \innerprod{ \mb a_i }{ \mb a_j } } \; \leq \; \mu ,\quad \frac{1}{n}\norm{ \mb a_i }{}^2 \;=\; 1, \;\; 1 \leq i \leq m.
%\end{align}
% Second, we assume that each entry of the dictionary $\mb A$ is i.i.d. random Gaussian. Notice that Assumption 2 is a special case of Assumption 1.
%\paragraph{Assumption 1: $\mu$-incoherent dictionary $\mb A$} For a given scalar $\eps$, we assume that
%\begin{align}\label{eqn:assump-incoherent}
%   \norm{\frac{1}{m} \mb A \mb A^\top - \mb I}{} \leq \eps , \qquad \max_{1\leq i,j\leq m, i\not = j} \abs{ \innerprod{\mb a_i}{\mb a_j} } \leq \mu n, \qquad \abs{ \norm{\mb a_i}{}^2 - n }\leq \eps, \; (1\leq i \leq m),
%\end{align}
%where the incoherence parameter $\mu \in \mc O\paren{ \sqrt{ \frac{ \log m }{m } } }$.

%\paragraph{Assumption 2: random dictionary $\mb A$}
%We assume that each component $\mb a_k$ of $\mb A$ is i.i.d. random Gaussian, 
%\begin{align*}
%   \mb a_k \sim_{i.i.d.} \mc N(0,1),\qquad 1\leq k\leq m.
%\end{align*}
%Note that this assumption is a special case of the previous one: with high probability over the randomness of $\mb A$, the conditions \eqref{eqn:assump-incoherent} hold for $\mb A$.  

%For the dictionary learning problem, we also make the following assumption for the sparse code $\mb X$.

%\paragraph{Sparse model of $\mb X$.} We assume that $\mb X$ follows the i.i.d. Gaussian-Bernoulli distribution with rate $\theta\in (0,1)$, i.e., $X_{ij}\sim_{i.i.d.} \mathrm{BG}(\theta)$ with
%\begin{align*}
%X_{ij} = B_{ij}G_{ij}, \quad B_{ij} \sim_{i.i.d.} \mathrm{Ber}(\theta), \quad G_{ij} \sim_{i.i.d.} \mc N(0,1),
%\end{align*}
%where $\theta \in (0,1)$ denotes the sparsity of $\mb X$. We write compactly $\mb X \sim_{i.i.d.} \mathrm{BG}(\theta)$.



